The Cost of Representation by Subset Repairs

Datasets may include errors, and specifically violations of integrity constraints, for various reasons. Standard techniques for ``minimal-cost'' database repairing resolve these violations by aiming for minimum change in the data, and in the process, may sway representations of different sub-populations. For instance, the repair may end up deleting more females than males, or more tuples from a certain age group or race, due to varying levels of inconsistency in different sub-populations. Such repaired data can mislead consumers when used for analytics, and can lead to biased decisions for downstream machine learning tasks. We study the ``cost of representation'' in subset repairs for functional dependencies. In simple terms, we target the question of how many additional tuples have to be deleted if we want to satisfy not only the integrity constraints but also representation constraints for given sub-populations. We study the complexity of this problem and compare it with the complexity of optimal subset repairs without representations. While the problem is NP-hard in general, we give polynomial-time algorithms for special cases, and efficient heuristics for general cases. We perform a suite of experiments that show the effectiveness of our algorithms in computing or approximating the cost of representation.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> section/dataset.tex <==
\section{Dataset}
In this section, we introduce the synthetic dataset designed for this task based on the Adult dataset.\footnote{We initially tried to work on real-life datasets including Adult, Hospital, Met, Voters, and German Credit. However, we had difficulties identifying proper functional dependencies with sensitive attributes.} In the proposed dataset, an adult has to fill in all his information, including age, work class, education, education-num, marital status, occupation, relationship, race, sex, hours per week, country, and income. We collect the information of 1100 adults as presented in the Holoclean repository. The functional dependency the dataset has to satisfy is that given the same education status, the education number must be the same, i.e.,
$$not(t1.Education=t2.Education\&t1.EduNum!=t2.EduNum)$$
Table~\ref{tab:Edu} indicates the corresponding mapping relations.
\begin{table}[t]
\centering
\small
{
\begin{tabular}{cc}
\textbf{Education} & \textbf{Education Number} \\ 
\toprule
Doctorate & 16 \\
Prof-school & 15 \\
Masters & 14\\
Bachelors & 13\\
Assoc-acdm & 12\\
Assoc-voc & 11\\
Some-college & 10\\
HS-grad & 9\\
12th & 8\\
11th & 7\\
10th & 6\\
9th & 5\\
7th-8th & 4\\
5th-6th & 3\\
1st-4th & 2\\
Preschool & 1 \\
\bottomrule
\end{tabular}
}
\caption{corresponding mapping relations between Education and EduNum.} 
\label{tab:Edu}
\end{table}

However, when filling out the information, people might correctly write down his/her education status, while choosing the wrong education number as there are 15 numbers to choose from. Our goal here is to repair the data we have collected to satisfy the abovementioned functional dependency. One assumption is that black woman with lower education level and the elderly is more likely to make such a mistake while filling in the information. As a result, if we conduct data repairing by deleting tuples to reach an optimal constrained set, we are more likely to delete tuples belonging to black women and the elderly, resulting in unfairness towards race, sex, and age.  We present the basic visualization of the dataset in Figure~\ref{fig:adult1}, Figure~\ref{fig:adult2} and Figure~\ref {fig:adult3}. We apply uniform sampling to choose 17 samples which might be a black woman with a lower education level or an elderly and assign an inconsistent education number for all these samples as a wrong sample \footnote{The full dataset can be referred to in this link: https://drive.google.com/file/d/1SZLtPwLPDXKg8ebck1EV9Qb-yANPe-Bj/view?usp=sharing}.
\begin{figure*}[t]
\centering
\scalebox{0.8}{
	
	\includegraphics[width=1\textwidth]{figure/adult1.png}}
	\caption{\label{fig:adult1}Analysis of sex and age. We can see from the figure that for the majority of men in the dataset is from 31 to 50 years old, while the majority of women in the dataset are 22-30 years old. However, we see that there are a certain amount of people both male and female in this dataset that can be defined as elderly who is older than 50, which leaves room for age unfairness.}
\end{figure*}

\begin{figure*}[t]
\centering
\scalebox{0.8}{
	
	\includegraphics[width=1\textwidth]{figure/adult2.png}}
	\caption{\label{fig:adult2}. Based on the data statistics, we can see that the races of males and females are proportionally balanced.}
\end{figure*}

\begin{figure*}[t]
\centering
\scalebox{0.8}{
	
	\includegraphics[width=1\textwidth]{figure/adult3.png}}
	\caption{\label{fig:adult3}.Based on the data statistics where the majority is white followed by black, we choose the black race as the potential unfairness group. }
\end{figure*}


We use Holoclean, a statistical inference probabilistic model to impute, clean, and repair data. We demonstrate the existence of unfairness by measuring the distribution shift of race (black), sex (female), and age (elderly) before and after data repair. After running the data repairing algorithm, we are able to identify all 17 wrong tuples and delete them to preserve the remaining 1083 as the optimal set. We present the distribution of sex in Table~\ref{tab:sex}. We can see that after data repair women have even fewer proportions as a minority proportion in the beginning, indicating the repairing algorithm doesn't maintain the distribution of sex and thus leads to sexual unfairness. We present the distribution of age in Table~\ref{tab:age}. We can see that the repairing algorithm doesn't maintain the distribution of age and thus leads to age unfairness. We present the distribution of race in Table~\ref{tab:race}. We notice a slight distribution change and the model is slightly unfair towards race\footnote{In some settings, these two distributions might be denoted as similar.}.

The proposed synthetic dataset has demonstrated that existing data repair tools, e.g., Holoclean with only optimal subset repair, don't take the distribution of sensitive attribute into account and thus suffers from bias. 


% \section{table}
\begin{table}[t]
\centering
\small
{
\begin{tabular}{lcc}
\toprule
Feature & Male & Female \\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5} \cmidrule(lr){6-6}
Before Data Repair & 0.68 & 0.32 \\
After Data Repair & 0.69 & 0.31 \\
\bottomrule
\end{tabular}
}
\caption{Calculated proportions of sex w and w/o optimal S-repair.} 
\label{tab:sex}
\end{table}
\begin{table}[t]
 \centering
\small
{
\begin{tabular}{lcc}
\toprule
Feature & Elderly (>50) & Young ($\leq$50) \\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5} \cmidrule(lr){6-6}
Before Data Repair & 0.18 & 0.82 \\
After Data Repair & 0.17 & 0.83 \\
\bottomrule
\end{tabular}
}
\caption{Calculated proportions of age w and w/o optimal S-repair.} 
\label{tab:age}
\end{table}
\begin{table}[t]
 \centering
\small
{
\begin{tabular}{lcc}
\toprule
Feature & Black & Other race \\
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5} \cmidrule(lr){6-6}
Before Data Repair & 0.086 & 0.914 \\
After Data Repair & 0.081 & 0.919 \\
\bottomrule
\end{tabular}
}
\caption{Calculated proportions of race w and w/o optimal S-repair.} 
\label{tab:race}
\end{table}


==> section/overview.tex <==
\section{Overview}
% The work by \cite{livshits2020computing} explores \subprob$(R, \Delta)$ and establishes its data complexity through a dichotomy. Specifically, if $\Delta$ can be reduced to an empty set by recursively applying three lossless simplifications based on \commonlhs{}, \consensusfd{} and \lhsmarriage{}, an optimal S-repair then can be computed in polynomial time. Otherwise, if this reduction is not feasible, \subprob$(R, \Delta)$ is proven to be NP-hard.

Our problem incorporates representation consideration into the procedure of data repairing. From the perspective of algorithms, we propose a collection of exact algorithms, approximations and heuristics to handle difference cases regarding to the input. They serve as the cornerstones of our theoretical results, shows the experimental observations and strengthens our primary motivations: 
\begin{itemize}
    \item Representation incurs an additional cost in database repairs, which our algorithm, based on integer linear programming (ILP), accurately estimates, even though this accuracy comes at the expense of scalability.
    \item By leveraging lossless simplifications, LP relaxations, intelligent rounding methods, and dynamic programming techniques, we can provide close-to-accurate estimates of this cost, along with corresponding representative S-repairs.
\end{itemize}

As the theoretical result, we establish a dichotomy (P, NP, and Unknown) for the data complexity of \prob$(R, \Delta, \rc{})$.
Specifically, we demonstrate that if \subprob$(R,\Delta)$ is NP-hard or $\dom{}(A_m)$ is not a constant, then \prob$(R, \Delta, \rc{})$ is also NP-hard. Conversely, if $\Delta$ is reducible to an empty set with simplifications based on \commonlhs s or \consensusfd s, \prob$(R, \Delta, \rc{})$ can be solved in polynomial time. However, when considering simplifications by \lhsmarriage s, we encounter a challenge, which we simplify into \skylineofmatching \yuxi{to change}. Nonetheless, even the complexity of the simplified version remains unknown, and we leave it along with the possibility of a polynomial-time algorithm (if feasible), as a future direction.

In our experiments, we introduce  baseline methods that combines existing repairing techniques with a post-cleaning procedure to enhance our findings. However, our objective is not to outperform these baselines, as their central objectives do not prioritize representation during the repairing procedure. Instead, we reinforce the accurate (or close-to-accurate) estimates generated by our algorithms and offer a range of representation-aware repair strategies, which encourage and inspires new ideas in the field of data cleaning. 

\yuxi{to change}
The remainder of this paper is organized as follows:
\begin{itemize}
    \item Section~\ref{sec:algorithm_all} presents all algorithms in detail,
    \item Section~\ref{sec:complexities} provides a summary of the complexity results,
    \item Section~\ref{sec:experiments} demonstrates our findings empirically.
\end{itemize}

% We prove that under this case, \prob$(R, \Delta, \mathcal{RC}_{R[A_m]})$ is NP-hard when the number of $A_m$'s distinct values $k$ is not constant. 

% We also present a randomized polynomial-time algorithm when every pair of values $(u,v)$ is distinct and the number of colors is constant. 


